The Case for Task Sampling based Learning for Cluster Job Scheduling

The ability to accurately estimate job runtime properties allows a scheduler to effectively schedule jobs. State-of-the-art online cluster job schedulers use history-based learning, which uses past job execution information to estimate the runtime properties of newly arrived jobs. However, with fast-paced development in cluster technology (in both hardware and software) and changing user inputs, job runtime properties can change over time, which lead to inaccurate predictions. In this paper, we explore the potential and limitation of real-time learning of job runtime properties, by proactively sampling and scheduling a small fraction of the tasks of each job. Such a task-sampling-based approach exploits the similarity among runtime properties of the tasks of the same job and is inherently immune to changing job behavior. Our study focuses on two key questions in comparing task-sampling-based learning (learning in space) and history-based learning (learning in time): (1) Can learning in space be more accurate than learning in time? (2) If so, can delaying scheduling the remaining tasks of a job till the completion of sampled tasks be more than compensated by the improved accuracy and result in improved job performance? Our analytical and experimental analysis of 3 production traces with different skew and job distribution shows that learning in space can be substantially more accurate. Our simulation and testbed evaluation on Azure of the two learning approaches anchored in a generic job scheduler using 3 production cluster job traces shows that despite its online overhead, learning in space reduces the average Job Completion Time (JCT) by 1.28x, 1.56x, and 1.32x compared to the prior-art history-based predictor.

==> Makefile-techreport-git <==
.SUFFIXES: .tex .dvi .ps .fig .eps .gnu .c
PDF = ps2pdf -dMaxSubsetPct=100 -dCompatibilityLevel=1.2 -dSubsetFonts=true -dEmbedAllFonts=true
CFLAGS  =  -Wall -g -Os -march=i686 -mpreferred-stack-boundary=2 -I/usr/local/include
CC =	gcc
LDFLAGS = -lm
.c:
	$(CC) -o $@ $(CFLAGS) $< $(LDFLAGS)


all: 	paper techreport cleanother


paper: paper.tex
	pdflatex --shell-escape paper
	pdflatex paper
	cp paper.pdf next.pdf
	cp paper.pdf ~/paper.pdf
	#scp next.pdf nescafe.ecn.purdue.edu:/data/ajajoo/Desktop/Research/jobScheduling/overleaf-slearn-paper/
	scp next.pdf min.ecn.purdue.edu:/home/min/a/ajajoo/figuresToDisplay/
	scp next.pdf moca.ecn.purdue.edu:/home/min/a/ajajoo/figuresToDisplay/

techreport: techreport.tex
	pdflatex --shell-escape techreport
	pdflatex techreport
	pdflatex techreport
	pdflatex techreport
	cp techreport.pdf techreport-slearn.pdf
	#scp next.pdf nescafe.ecn.purdue.edu:/data/ajajoo/Desktop/Research/jobScheduling/overleaf-slearn-paper/
	scp techreport-slearn.pdf min.ecn.purdue.edu:/home/min/a/ajajoo/figuresToDisplay/
	scp techreport-slearn.pdf moca.ecn.purdue.edu:/home/min/a/ajajoo/figuresToDisplay/

#	scp paper.pdf nescafe:~/Desktop/CN18-paper.pdf
#	gnome-open paper.pdf >out.out 2>err.err 

#	bibtex paper


#	dvips -Pdownload35 -t letter -o paper.ps paper.dvi
#	$(PDF) paper.ps

#	bash -c 'if [[ -f .Zheng ]]; then acroread paper.pdf; else ggv paper.ps; fi'
#	dvips -Pcmz  -t letter -o paper.ps paper.dvi
#	dvips -Pcmz  -t letter -o paper.ps paper.dvi
#	bibtex paper
#	sed -e 's/\(\\begin{thebibliography}{.*}\$\)/\1\\medskip/g' paper.bbl > paper.bbl.mv && mv paper.bbl.mv paper.bbl

bib:	
	pdflatex paper
	pdflatex paper
	bibtex paper
	#bibtex paper
	pdflatex paper
	pdflatex paper
	
	pdflatex techreport 
	pdflatex techreport 
	bibtex techreport 
	pdflatex techreport 
	pdflatex techreport 

sub:
	./submit.sh

aj: all 
	scp next.pdf min.ecn.purdue.edu:/home/min/a/ajajoo/figuresToDisplay/
	#scp next.pdf nescafe:~/Desktop/nextPaper.pdf
	#scp esys20.pdf nescafe:~/Desktop/ESYS20-paper.pdf
	#scp socc19.pdf nescafe:~/Desktop/SOCC19-paper.pdf
	#scp atc19.pdf sp13:~/Desktop/ATC19-paper.pdf

clean: cleanother cleanbib
	rm -rRf *.pdf

cleanother:
	rm -rRf *.dvi *.aux *.blg *.log *.ps *~ paper.out
	
cleanbib:
	rm -rRf *.bbl

cleanotherandout: cleanother cleanout

cleanmajor: clean cleanout

cleanout:
	rm -rRf *.out

fresh : clean bib paper

freshaj : fresh
	scp next.pdf nescafe:~/Desktop/nextPaper.pdf
	#scp socc19.pdf nescafe:~/Desktop/SOCC19-paper.pdf
	#scp atc19.pdf sp13:~/Desktop/ATC19-paper.pdf


==> backg.tex <==
\section{Challenges in Scheduling Big-Data Jobs}
\label{sec:back}
 
\subsection{Background}
\label{subsec:back}
 
Clusters are being shared among multiple users to execute diverse
jobs that arrive online. 
%Such jobs typically arrive online and compete for shared resources. 
In order to best utilize the cluster and to ensure that
jobs also meet their service level objectives (SLOs), efficient job
scheduling is essential. Since jobs arrive online, their runtime
properties, such as task running-times, network flow sizes, 
memory and disk IO requirements,
%or \emph{runtime} for short,
%characteristics 
are unknown \emph{a priori}. This lack of information 
%about job runtime properties 
poses a fundamental challenge to the scheduler in trying to determine
the right order of job execution that would meet application SLOs
%service level objectives (SLOs) 
and/or maximize the utilization of shared hardware resources.
 
\subsection{Problem Statement}
 
\paragraph*{Job Model.}
Formally, we consider typical big-data jobs in a shared cluster (either
private or public), where each big-data job processes a large amount of
data. Each job partitions the data into manageable chunks and runs many
parallel tasks (which we refer to as \emph{compute tasks}), one for processing each data chunk. 
%to achieve
%specific SLO such as minimizing the completion time or meeting some
%deadline. 
Compute tasks may also exchange intermediate results, which we refer to as
\emph{network tasks}. 
%
Examples of such big-data jobs may involve a single phase of parallel
compute tasks (e.g., in the mapper stage of MapReduce) or network tasks
(also known as the co-flow
problem~\cite{coflow:hotnets12,aalo:sigcomm2015,
varys:sigcomm14,baraat:sigcomm14, graviton:hotcloud16,
jajooSaath,jajoo:atc2019}), or multiple phases of compute and network
tasks with dependency modeled by
directed acyclic graphs (DAGs)~\cite{mapreduceonline:nsdi2010,
apache:tez, dryad:eurosys2007, dandelion:sosp2013}.

In developing various approaches to big-data job scheduling in this
proposal, we first focus on a single phase of parallel tasks. Our
job model of a single phase of parallel tasks is similar to that of
~\cite{borg,perforator:socc2016,IfYouAreLateDontBlameUs:socc14} and
forms the building block for generalized job scheduling strategies
that schedule multi-phase (DAG) jobs (see  Task~6).
 
\paragraph*{Scheduling Objectives.}
Different jobs can have different application SLOs. For some jobs meeting
deadlines is more important while for others faster job completion
time or minimizing the use of data center resources such as networks
is more important. Such a diverse set of objectives pose further
challenges in scheduling big data-jobs in shared
clusters~\cite{drf:nsdi11,jockey:eurosys2012, shufflewatcher, corral,
  morpheus, delay:eurosys10, cdef:atc18}.
 
\subsection{Prior-Art}
\label{subsec:prior}
 
\paragraph*{History-based Learning.}
An effective way to tackle the challenges of cluster scheduling is to
learn and estimate runtime characteristics of pending
jobs. Intuitively, if we can accurately estimate jobs characteristics,
we can leverage offline 
scheduling algorithms for minimizing the average completion time, e.g.,
SJF (shortest-job-first) is known to optimal for certain settings.
 
The problem of learning runtime characteristics of jobs has been
intensively studied. Cluster schedulers using various learning methods
have been proposed~\cite{corral, morpheus, shufflewatcher, 3Sigma,
  tetrisched, DontCryOverSpilledRecords, perforator:socc2016,
  Apollo:osdi2014, wsmith:IEEE98, stratus:socc2018,
  roughSetEstimation:IEEE:Shonali}.  All previously proposed learning
schemes, however, are history-based, i.e., they learn job characteristics by
observations made from the past job executions. 
%  In particular, existing history-based learning approaches can be broadly categorized
% into the following groups, 
% as summarized in Table 1.

\paragraph*{Limitations of History-based Learning.} Accurately predicting job runtime
characteristics from history information relies on two conditions to
hold: (1) Most of the jobs are recurring; (2) The performance of the
same or similar jobs will remain consistent over time. In the
following, we argue why these conditions may not be applicable to
modern-day clusters.
 
{\em Condition 1: Most of the jobs are recurring.}  Many previous work
have acknowledged that not all jobs are recurring. For example, the
traces used in Corral~\cite{corral} and Jockey~\cite{jockey:eurosys2012} show that only 40\% of the jobs are
recurring and Morpheus~\cite{morpheus} shows that 60\% jobs are
recurring.

{\em Condition 2: The performance of the same or similar job will remain
consistent over time.}
Previous works~\cite{3Sigma, morpheus, corral, jockey:eurosys2012} that exploited
history-based prediction have considered jobs in one of
the following two categories.
%\begin{itemize}
(1) {\em Recurring jobs}: A job is re-scheduled to run on newly arriving data;
(2) {\em Similar jobs:} A job has not been seen before but has some
attributes in common with some jobs executed in the past. The
attributes can be application name, job name, user of
the job, or amount of resources requested by the job.
%\end{itemize}
Many of the history-based approaches only predict for recurring jobs \cite{morpheus, corral,
jockey:eurosys2012}, while some others \cite{3Sigma, jamiasvu, stratus:socc2018, roughSetEstimation:IEEE:Shonali} work for both categories of jobs.
%
However, \emph{even the authors of history-based prediction schemes such as
3Sigma~\cite{3Sigma} and Morpheus~\cite{morpheus} strongly argued why
runtime properties of jobs, even with the same input, will not remain consistent
and will keep evolving.}  The primary reason is that updates in cluster
hardware, application software, and user scripts to execute the jobs
all affect the job runtime characteristics.
{They found that}
in a large Microsoft production cluster, within a one-month period,
applications corresponding to more than 50\% of the recurring jobs were
updated. The source code changed by at least 10\% for applications
corresponding to 15-20\% of the jobs.  Additionally, over a one-year period,
the proportion of two different types of machines in the cluster
changed from 80/20 to 55/45. For a same production Spark job, there is
a 40\% difference between the running times observed on the two types of
machines~\cite{morpheus}. 
%\linx{Does Spark mean streaming jobs? I think
%our approach does not apply for streaming jobs.}

For these reasons, although the state-of-the-art job scheduling system 3Sigma~\cite{3Sigma} 
uses sophisticated history-based prediction techniques,
% Machine Learningd also shown that
the predicted running times for more than 23\% of the jobs have at
least 100\% error, and for many the prediction is off by an order of
magnitude. In our experiments with production cluster traces (see
Fig.~\ref{fig:sim:estimationAccuracy:2STrace}), we observed similar
levels of high variability in the runtime characteristics of the jobs with the same
attributes.

%\linx{How about adding a paragraph for "Non-Learning Based Approaches".
\paragraph*{Non-learning-based approach.}
Using priority queues to adaptively adjust the priority of a
distributed job based on how long it has run
(which is related to age-based
scheduling policies such as Least Attained Service~\cite{scully2018soap,raiLAS:sigmetrics2003})
% and the principle of Least Attained Service~\cite{raiLAS:sigmetrics2003}. 
has been explored for both network tasks
(i.e., coflow scheduling)~\cite{aalo:sigcomm2015,graviton:hotcloud16,jajooSaath} and
compute tasks~\cite{kairos:socc2018}.
While these
approaches also adapt to real-time feedback, they do not aim to
explicitly learn job characteristics from completed tasks, and thus are
fundamentally different from the online learning approach that we
propose below.  As a result, they adapt more slowly and tend to
degrade to round-robin scheduling when jobs are of similar
sizes~\cite{jajoo:atc2019}.

%% 2.3.2 Scheduling without online learning
 
%\linx{I can write a paragraph here to introduce the key new concept of online learning.}
 




\if 0

\paragraph*{Scheduling Objectives.}

%\newline 

\linx{The following paragraph may goes to the end of ``background section''}

\paragraph*{Online Learning:} In this project, we propose a new
online-learning based approach to the scheduling and optimization of
big-data clusters. In a typical online learning problem (such as
multi-armed bandit \cite{MAB}), the controller faces significant
uncertainty in key parameters of the problem (such as the expected
payoff of each arm). Thus, the controller must use feedback from past
control decisions to learn, and gradually refine, the knowledge of these
parameters, while making control decisions that utilize the learned
knowledge at the same time. This integration of learning and control is
a natural fit for big-data cluster scheduling: since the multiple
compute and network tasks of a job often share similar characteristics, 
the feedback from
completed tasks can be used to learn the underlying
features of the entire job, which can then be used to make more informed
scheduling decisions. In Section~\ref{}, we will present 
preliminary evidence demonstrating that this new concept can
lead to significant performance gains over
existing approaches. 
%history-based appraoches and approaches without learning. 
However, as we will elaborate in the rest of the proposal, existing
theoretical results and algorithms on online learning often cannot be
directly applied here.
First, existing online learning problems usually focus on
payoff-maximization \cite{MAB}, while we care about computer-system objectives such
as completion time and throughput. This difference in control objectives
has a direct impact on what are the most important parameters to learn,
how to learn them, and how to utilize the learned parameters at
different confidence levels. Thus, both the learning and control
component must be carefully redesigned in an integrated manner. 
Second, existing online learning problems often focus on a snapshot
problem with a fixed set of agents and choices \cite{snapshot}, while in
a cluster jobs keep arriving and departing. This calls for the
integration of online
learning with stochastic control, which also presents significant new
difficulty. 
%only received few attention in the literature. 


\fi


==> comparison-techreport.tex <==
\section{Accuracy Analysis}
\label{sec:accuracy}
% 1. Write about using training data as best of the history here and in \S\ref{sec:study}.\\ 
% 2. Argument for using the 2Sigma trace as the main
% evaluation trace and other answers about the trace diversity here and in
% \S\ref{sec:study}.}

In this section, we perform an in-depth study of the prediction
accuracy of the two learning approaches: {\em learning in time}
(history-based learning) and {\em learning in space}
(task-sampling-based learning).  
{
Both approaches can potentially be used
to learn  different job properties for different optimization objectives.
In this paper, we focus on job completion time 
because it is an important metric that has been intensively studied
in recent work~\cite{cora:infocom2015,DontCryOverSpilledRecords,kairos:socc2018,varys:sigcomm14,corral,3Sigma,AltruisticScheduling,aalo:sigcomm15}.
}


We first derive analytical bounds on
their prediction errors (\S\ref{sec:accuracy:quantity}).  We then
measure and compare the bounds in real traces from two production
datacenters (\S\ref{sec:accuracy:trace}).  Finally, we
experimentally compare the prediction accuracy of learning in space
with a history-based predictor
\primarybasepredict~\cite{3Sigma} in estimating the job runtimes
(\S\ref{sec:accuracy:experiment}).
We pick \primarybasepredict because it is a state-of-the-art 
history-based predictor that can learn for non-recurrent jobs.

%  , and thus specific choices are somewhat orthogonal to the main focus of our
%  paper, which is to show that sampling-based prediction can be a viable
%  alternative to history-based prediction, explain the situations where
%  it will work well, and demonstrate its effectiveness empirically
%  through production traces. 
% Consistent with this objective, we mainly focus on estimating task running-times.

\vspace{-0.1in}
\subsection{Quantitative Comparison}
\label{sec:accuracy:quantity}

We first  present a theoretical analysis to compare the two
approaches. We caution that here we use a highly-stylized model (e.g., two
jobs and normal task-length distributions), which does not capture the
possible complexity in real clusters, such as heavy parallelism across servers and highly-skewed 
task-length distributions. Nonetheless, it reveals important insights
that help us understand in which regimes history-based schemes or sampling-based
schemes will perform better. Consider a simple case of two jobs
$j_1$ and $j_2$, where each job has $n$ tasks. The size of each task of $j_1$
is known. Without loss of generality, let us assume that the task size of $j_1$
is 1. Thus, the total size of $j_1$ is $n$. The size of a task of $j_2$ is
however unknown.
% Instead, we know the following about $j_2$: 
%  \editaj{(1) The average
%  task size across all tasks of $j_2$, denoted by $x$, follows a normal
%  distribution with mean $\mu$ and variance $\sigmanotsqrd$;}{
Let $x$ denote the average task size of $j_2$, and this its total size
is $n x$. Clearly, if we knew $x$ precisely, then we should have
scheduled $j_1$ first if $x > 1$ and $j_2$ first if $x \le
1$. However, suppose that we only know the following:
(1) % The average task size of $j_2$, denoted by
(Prior distribution:) $x$ follows a normal
distribution with mean $\mu$ and variance $\sigmanotsqrd$;
(2) Given $x$, the size of a random task of the job follows a normal 
distribution with mean $x$ and variance $\sigmaonesqrd$.
Intuitively, $\sigmanotsqrd$ captures the variation of mean
task-lengths \emph{across} many \emph{i.i.d.} copies of job $j_2$,
\ie job-wise variation,
while $\sigmaonesqrd$ captures the variation of task-lengths \emph{within} a
single run of job $j_2$,
\ie task-wise variation.
% \soccReviewEdit{A}{
We note that the parameters $\sigmanotsqrd$ and
$\sigmaonesqrd$ are used below to understand the accuracy of both
history-based and sampling-based predictors, whose goal is to estimate
the mean task-length $x$ (and consequently the job runtime which equals
$x$ times the number of tasks)
of a new copy of job $j_2$. The predictors
themselves may not use the knowledge of $\sigmanotsqrd$ and
$\sigmaonesqrd$. In practice,
these parameters can be estimated offline from historical data. 
We will see soon that the performance of history-based schemes
will mainly depend on $\sigmanotsqrd$, while the performance of sampling-based
schemes will mainly depend on $\sigmaonesqrd$.
%}

%In practice, all these parameters can be obtained from historical data.
%Specifically, $\sigmanotsqrd$ can be estimated from the data of mean
%task-lengths (each of which is an average among the tasks in a job) across jobs,
%while $\sigmaonesqrd$ can be estimated from the data of task-lengths among
%the tasks of the same job. Thus, we will refer to $\sigmanotsqrd$ and
%$\sigmaonesqrd$ as the {\em job-wise variations} and {\em task-wise variations},
%respectively. 
%We will see soon that the performance of history-based schemes
%will mainly depend on $\sigmanotsqrd$, while the performance of sampling-based
%schemes will mainly depend on $\sigmaonesqrd$.

%\todoaj{Discuss with prof. Lin and write following claims in a better way.\\}
%We will show that:\\
%(1) if $\sigmanotsqrd >> \sigmaonesqrd$, sampling will be effective.\\
%(2) if $\sigmanotsqrd << \sigmaonesqrd$, sampling will not be very effective.\\

Towards this end, let us consider two options: (1) A history-based approach
(\S\ref{sec:accuracy:quantity:history}) and (2) a sampling-based approach where
we sample $m$ tasks from $j_2$ (\S\ref{sec:accuracy:quantity:sampling}).

\subsubsection{History-based Schemes}
\label{sec:accuracy:quantity:history}
Since no samples of job $j_2$ are used, the best predictor for its mean task
length is $\mu$.
In other words, the scheduling decision will be based on $\mu$ only. The difference between the
true mean task length, x, and $\mu$ is simply captured by the job-wise variance
$\sigmanotsqrd$.

%If $\mu>1$, then $j_1$ should
%go first. The total completion time in this case is $n(1+(1+\mu))$.  Now if
%$\mu<1$, then $j_2$ should go first. The total completion time in this case
%will be $n(\mu+(\mu+1))$.  So in both cases, the total completion time is
%\footnote{For sake of simplicity in analysis we have assumed that there is only one server.}:
%\begin{equation}
%\label{equation:historyExpectation}
%n(1+\mu+min(1,\mu))
%\end{equation}

\subsubsection{Sampling-based Schemes}
\label{sec:accuracy:quantity:sampling}
Suppose that we sample $m$ tasks from $j_2$. Collect the sampled task lengths into a vector:
\begin{center}
	$\yvec = \left( y_1, y_2, ..., y_m \right)$.
\end{center}
Then, based on our probabilistic model, we have
\begin{center}
	$P\left(y_i|x\right) = \frac{1}{\sqrt{2\pi}\sigmaone}e^{-\frac{\left(y_i - x\right)^2}{2\sigmaonesqrd}}$\\
	$P\left(\yvec|x\right) = {\prod_{i=1}^{m}}\frac{1}{\sqrt{2\pi}\sigmaone}e^{-\frac{\left(y_i - x\right)^2}{2\sigmaonesqrd}}$
\end{center}
We are interested in an estimator of $x$ given $\yvec$. We have 
%%\commentaj{added a footnote here.}\footnote{
%\soccReviewEdit{A}{
%%We do not include the detailed derivation here due to space limit. However, it is 
%}
%$P\left(x|\yvec\right)$
\begin{center}
	$P\left(x|\yvec\right) = \frac{P\left(\yvec|x\right)\cdot P(x)}{P(\yvec)} = \frac{P(\yvec|x)\cdot P(x)}{\int_{x}P(\yvec|x)\cdot P(x)dx}$

	$= \frac{1}{\sqrt{2\pi}}\left[\frac{m}{\sigmaonesqrd} +
	\frac{1}{\sigmanotsqrd}\right]^\frac{1}{2} \cdot e^{-
	\left(\frac{m}{2\sigmaonesqrd} +
	\frac{1}{2\sigmanotsqrd}\right)\left(x -
	\frac{{\sum_{i=1}^{m}\frac{1}{\sigmaonesqrd}y_{i} +
	\frac{1}{\sigmanotsqrd}\mu}}{\frac{m}{\sigmaonesqrd} +
	\frac{1}{\sigmanotsqrd}}\right)}$,
\end{center}
where the last step follows from standard results on the posterior distribution
with Gaussian priors (see, \eg~\cite{jordanLecturePosterirorDistribution}).
%This confirms that $x|\yvec$ is also a normal distribution with:\\
In other words, conditioned on $\yvec$, $x$ also follows a normal distribution with
mean = $ \frac{{\sum_{i=1}^{m}\frac{1}{\sigmaonesqrd}y_{i} + \frac{1}{\sigmanotsqrd}\mu}}{\frac{m}{\sigmaonesqrd} + \frac{1}{\sigmanotsqrd}}$ 
and variance = $\frac{1}{\frac{m}{\sigmaonesqrd} + \frac{1}{\sigmanotsqrd}}$.

Note that this represents the estimator quality using the information of
both job-wise variations and task-wise variations. If the estimator
% ignores
is not informed of the
job-wise variations, we can take $\sigmanotsqrd  \rightarrow +\infty$, and
the conditional distribution of $x$ given $\yvec$ becomes normal with mean
$\frac{1}{m} \sum_{i=1}^{m} y_{i}$ and variance $\frac{\sigmaonesqrd}{m}$.

From here we can draw the following conclusions. First, whether history-based
schemes or sampling-based schemes have better prediction accuracy for an unknown
job depends on the relationship between job-wise variations $\sigmanotsqrd$ and
the task-wise variation $\sigmaonesqrd$. If the job-wise variations are large
but the task-wise variation is small, \ie $\sigmanotsqrd >>
\frac{\sigmaonesqrd}{m}$, then sampling-based schemes will have better
prediction accuracy. Conversely, if the job-wise variations are small but
the task-wise variation is large, \ie $\sigmanotsqrd <<
\frac{\sigmaonesqrd}{m}$, then  history-based schemes will have better
prediction accuracy. Second, while the accuracy of history-based schemes is
fixed at $\sigmanotsqrd$, the accuracy of sampling-based schemes improves as $m$
increases. Thus, when we can afford the overhead of more samples, the
sampling-based schemes become favorable. Our results from experimental
data below will further confirm these intuitions.

\if 0

So, now once sampling is done we can make decision based on:\\
\begin{center}
\xspace $\mathbb{E}[x|\yvec] \cdot (n-m)$. 
\end{center}
If $\mathbb{E}[x|\yvec](n-m) > n$, then $j_1$ should be scheduled first otherwise $j_2$.
The total completion time in this case will be:\\
$Z = \sum_{i=1}^{m} y_{i} + \mathbb{E}(x|\yvec)(n-m) + n + min[\mathbb{E}(x|\yvec)(n-m), n]$\\
and the expected total completion time will be:\\
\begin{equation}
\label{equation:samplingExpectation}
\mathbb{E}(Z) = n\cdot\mu + n + \mathbb{E}\left[ min\left(\frac{{\sum_{i=1}^{m}\frac{1}{\sigmaonesqrd}y_{i} + \frac{1}{\sigmanotsqrd}\mu}}{\frac{m}{\sigmaonesqrd} + \frac{1}{\sigmanotsqrd}}\cdot(n-m),n\right)\right]\\
\end{equation}
\fi

\if 0
\begin{figure}[tp] 
\centering
\subfigure[\vspace{-0.2in} sigma0 = 0.01 sigma1 = 1]
{
\includegraphics[width=0.9\linewidth]{figures/numerical_analysis/numerical_analysis_0pt5_1pt5_0pt01_sigma0-0pt01_sigma1-1_varying_mu.pdf}
\label{fig:numerical_analysis:variableMu}
}
\subfigure[\vspace{-0.2in} sigma0 = 1 sigma1 = 0.01]
{
\includegraphics[width=0.9\linewidth]{figures/numerical_analysis/numerical_analysis_0pt5_1pt5_0pt01_sigma0-1_sigma1-0pt01_varying_mu.pdf}
\label{fig:numerical_analysis:variableMu}
}
\caption{Numerical Analysis. Varying $\mu$ from 0.5 to 1.5 with step of 0.01. $m = 5$, $n = 100$.
	\todoaj{Make the y-label as "E[Total JCT]"}
	}
\vspace{-0.1in}
\label{fig:qunatitative_analysis}
\end{figure}
\fi

%\if 0
\begin{table}[tp]
\caption{Summary of trace properties.}
\label{table:traceSummary}
\centering
{\small
\vspace{-0.1in}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
		\textbf{ Trace} & \textbf{Arrival} & \textbf{Resource} & \textbf{Resource}  & \textbf{Indiv. task} \\
			& \textbf{time} & \textbf{requested} & \textbf{usage} & \textbf{duration}\\
 
\hline
	  \textbf{2Sigma} & Yes & Yes & No & Yes\\
\hline
	  \textbf{Google 2011} & Yes & Yes & Yes & Yes\\
\hline
	  \textbf{Google 2019} & Yes & Yes & Yes & Yes\\
\hline
%\hline
%		\textbf{ Trace} & \textbf{Arrival} & \textbf{Resource} & \textbf{Resource}  & \textbf{Individual} & \textbf{Task success}&{\bf Fraction of}\\
%			& \textbf{time} & \textbf{requested} & \textbf{usage} & \textbf{task duration} & \textbf{status} &{\bf thin jobs}\\
%	 
%\hline
%	  \textbf{2Sigma~\cite{2Sigma:trace}} & Yes & Yes & No & Yes & Yes & Relatively low\\
%\hline
%	  \textbf{Google~\cite{googleTraceGithub}} & Yes & Yes & Yes & Yes & Yes & Relatively High\\
%\hline
\end{tabular}
\vspace{-0.1in}
}
\end{table}
%\fi


\subsection{Trace-based Variability Analysis}
\label{sec:accuracy:trace}


Our theoretical analysis in \S\ref{sec:accuracy:quantity} provides 
insights on how the prediction accuracies of the two approaches depend
on the variation of job run times across time and space.
To understand how such variations fare against each other in practice,
we next measure the actual variations
%  in average task runtimes for jobs across history ($\sigmanotsqrd$) and in task
%  runtime across the tasks of the same job (${\sigmaonesqrd}$).
in three production cluster traces.

%  %  , one from 2Sigma~\cite{2Sigma:trace} and
%  two from Google~\cite{googleTraceGithub, googleClusterData2019},
%  released in 2011 and in 2019, respectively.

\if 0
Several previous work have experimented to
measure variation across history \cite{morpheus, corral, 3Sigma,
jockey:eurosys2012}. We use the technique based on the state-of-the-art
predictor 3Sigma-Predict~\cite{3Sigma}.
\fi

%\paragraph{Traces.} The Google trace is a publicly
%available~\cite{googleTraceGithub}, 29-day long trace
%collected in May 2011 from a Borg~\cite{borg} cell on a cluster of
%approximately 12.5K machines.
%The machines  are highly heterogeneous; 
%they belong to at least
%three different platforms which use different micro-architectures and/or
%memory technologies~\cite{workloadDiversity:atc18}, and
%according to~\cite{googleClusterData2011-2Schema},
%the machines in the same platform can have substantially different clock rates,
%memory speed, and core counts.
%%It has complete information for more than 0.67 million jobs.
%(The trace does not contain actual machine properties. Other details can be
%found in~\cite{googleClusterData2011-2Schema,googleTraceGithub}).
%The second trace is collected from a private datacenter of 2Sigma. The
%cluster uses an internal proprietary job scheduler running on top of a {Mesos
%cluster manager}~\cite{2Sigma:scheduler}. This trace was collected for a period of 7
%months and from  872 machines. The entire trace contains
%approximately 0.4 million jobs.
%    Table \ref{table:traceSummary} summarizes the information available in the traces.
%  that are used in our analysis.
%
%We calculate the variations in task
%runtimes for each job across time and across space as follows.
%Corresponding to each job, we calculate the following 2 values (a)
%Coefficient of variation (CoV) in average task runtimes across time 
%observed at the time of job arrival and, (b) Observed CoV in task runtimes of the job.

\paragraph{Traces.} 
%
Our first trace is provided by 2Sigma~\cite{2Sigma:website}.
% engineers collected from their cluster.
The cluster uses an internal proprietary job scheduler
running on top of a {Mesos cluster manager}~\cite{2Sigma:scheduler}. This trace
was collected over a period of 7 months, {in July 2016}, and from  441
machines and contains approximately 0.4 million jobs ~\cite{2Sigma:trace}.
Table~\ref{table:traceSummary} summarizes the information available in the
traces that are used in our analysis.

We also include two publicly available traces from Google released in
May 2011 and May 2019~\cite{googleTraceGithub, googleClusterData2019},
collected from 1 and 8 Borg~\cite{borg} cells
over periods of 29 and 31 days, respectively.  The machines in the clusters are
highly heterogeneous, belonging to at least three different
platforms that use different micro-architectures and/or memory
technologies~\cite{workloadDiversity:atc18}. Further, according
to~\cite{googleClusterData2011-2Schema}, the machines in the same
platform can have substantially different clock rates, memory speed,
and core counts.
%   (The trace does not contain actual machine
%   properties. Other details can be found
%   in~\cite{googleClusterData2011-2Schema, googleClusterData2019}).
%  As mentioned in~\cite{borgTraceAnalysis2019}, Google 2019 trace is very
%  large and has 2.8 TiB in compressed form and hence Google made it
%  available only via \textit{bigquery}~\cite{web:googleBigquery}.
%  First, the Google
%    2019 trace had information about the job tier, \eg batch or
%    production. Since the SLO for batch tier jobs is to minimize the
%    average completion time, we chose batch tier jobs from the 2019
%    trace.  Second,
Since the original Google 2019 trace has data from 8 different
cells located in 8 different locations,
%  . From private
%    communication~\cite{personalCommunication:Nan} we learned that {at
%      Google, the job properties vary with the social behaviour of
%      different locations and it is hard to identify an average cell.
and given that we already have two other traces from the US, we chose 
the batch tier of {Cluster G} in the Google 2019 trace, which is located in
Singapore~\cite{googleClusterData2019Schema}, as our third trace to
diversify our trace collection.


\if 0
Google has publicly released two sets of traces, one collected
in May 2011 and another in May 2019~\cite{googleTraceGithub,
  googleClusterData2019}.  The traces have information collected over
a period of 29 (31) days from 1 (8) Borg~\cite{borg} cells for the
2011 (2019) trace and are released in csv (bigquery) format.  The
machines are highly heterogeneous; they belong to at least three
different platforms which use different micro-architectures and/or
memory technologies~\cite{workloadDiversity:atc18}, and according
to~\cite{googleClusterData2011-2Schema}, the machines in the same
platform can have substantially different clock rates, memory speed,
and core counts.  (The trace does not contain actual machine
properties. Other details can be found
in~\cite{googleClusterData2011-2Schema, googleClusterData2019}).  As
mentioned in~\cite{borgTraceAnalysis2019}, Google 2019 trace is very
large and has 2.8 TiB in compressed form and hence Google made it
available only via \textit{bigquery}~\cite{web:googleBigquery}.
\fi 


We calculate the variations in task runtimes for each job across time and
across space as follows.

\paragraph{Variation across time.} To measure the variation in mean task
runtime for a job across the history, we follow the following prediction
mechanism defined in 3Sigma~\cite{3Sigma} to find similar jobs.

As discussed in \S\ref{sec:back:existing}, 3Sigma~\cite{3Sigma} uses
multiple features to identify a job and predicts its runtime using the feature
that gives the least prediction error in the past. We include all six features
used in 3Sigma:
{application name}, {job name}, {user name}
(the owner of the job), {job submission time (day and hour)},
and {resources requested} by the job.
%These are the same set of features as listed in 3Sigma~\cite{3Sigma}.  

% hitory. However, they approximate it as storing entire history will take too much memory.}
For each feature, we define the set of similar jobs as
all the jobs executed in the history window
(defined below) that had the same feature value.
Next, we calculate the average task runtime of each job in the set. Then, we
calculate the {\em Coefficient of Variation} (CoV) of the average task runtimes
across all the jobs in the set. We repeat the above process for all the
features.  We then compare the CoV values thus calculated and pick the minimum
CoV.
% The above procedure is similar in
% principle to the prediction procedure of 3Sigma~\cite{3Sigma}.
Effectively, the above procedure selects the least possible variation
across history.

\paragraph{Varying the history length in prediction across time.}
%\questionaj{The figure \ref{fig:accuracy:trace} is on job count
%window. Will add a day wise figure for \ref{fig:accuracy:trace} too. But there
%we need to have only one fixed window size. We cannot have multiple windows
%there. What do you think we should keep the window size?}
3Sigma used the entire history for prediction.
Intuitively, the length of the history affects the trade-off between
the number of similar jobs and the staleness of the history information.
For this reason, we optimized 3Sigma
by finding and using the history length that gives the least variation.
Specifically, we define the length of history based
on a window size $w$, \ie the number of past consecutive days.
%  In particular, when we calculate the CoVs for a job on day $i+w$,
% the history window starts from day $i$ to day $i+w-1$.
In our analysis below, we vary $w$ among 3, 7, and 14 for the
three traces.
% Google 2011 and 2019 traces.
% 3, 7, and 14 for the 2Sigma trace.

%   Next, we calculate CoVs in the same way as described
%   above for all the jobs on $i+w+1^{th}$ day using all the jobs in range $i^{th}$
%   to $i+w^{th}$ day as the training data. For each value of $w$ we adjust $i$ such
%   that the set of end days \ie set of $i+w+1^{th}$ days is same for all the three
%   window sizes.
%For one window period we plot one CDF of all the CoVs measured by
%varying the window over it's range. The space curve shows the task CoV.
%$\sqrt{numberOfTasks*0.05}$

\if 0
\begin{figure*}[tp]
%\vspace{-0.1in}
\centering
\subfigure[Task runtime -- 2Sigma]
{
\includegraphics[width=0.2\linewidth]{figures/trace_analysis/slidingWindow_analysis_unified_cdf_of_covs_in_avg_task_runtime_for_user_name_in_2Sigma.pdf}	% done
\label{fig:accuracy:trace_analysis_window:2Sigma:task_dur}
}
\hspace{-12pt}
\subfigure[Task runtime -- Google 11]
{
\includegraphics[width=0.2\linewidth]{figures/trace_analysis/slidingWindow_analysis_unified_cdf_of_covs_in_avg_task_dur_for_application_name_in_google11.pdf}	% done
\label{fig:accuracy:trace_analysis_window:google11:task_dur}
}
\hspace{-12pt}
\subfigure[Task runtime -- Google 19]
{
\includegraphics[width=0.2\linewidth]{figures/trace_analysis/slidingWindow_analysis_unified_cdf_of_covs_in_avg_task_dur_for_application_name_in_google19.pdf}	% done
\label{fig:accuracy:trace_analysis_window:google19:task_dur}
}
\hspace{-12pt}
\vspace{-0.1in}
\subfigure[CPU usage -- Google 11]
{
\includegraphics[width=0.2\linewidth]{figures/trace_analysis/slidingWindow_analysis_unified_cdf_of_covs_in_mean_CPU_usage_for_application_name_in_google11.pdf}	% done
\label{fig:accuracy:trace_analysis_window:google11:cpuUsage}
}
\hspace{-12pt}
\subfigure[Disk IO time -- Google 11]
{
\includegraphics[width=0.2\linewidth]{figures/trace_analysis/slidingWindow_analysis_unified_cdf_of_covs_in_mean_diskIO_time_for_application_name_in_google11.pdf}	% done
\label{fig:accuracy:trace_analysis_window:google11:diskIO}
}
\vspace{-0.1in}
\caption{CDF of CoV of runtime properties 
  across space
  and across time with varying history windows,
          using the 2Sigma, Google 2011 and Google 2019 traces.
%%	  Single-task jobs are excluded from the analysis across space.
%          Figures show coefficient of variation in
%	measured runtime properties of the job. For measuring CoV across time
%	(history) we choose the feature with least variation as described in
%	\S\ref{sec:accuracy:trace}. Also, in case of time we plot the average
%	value of the property of the tasks of a job. For space we plot CoVs
%	across tasks of the job as described in \S\ref{sec:accuracy:trace}. In
%	this analysis we excluded single task jobs. The CDFs are for all the
%	jobs in the window period.Figure
%	\ref{fig:accuracy:trace_analysis_window:google11:cpuUsage} and
%	\ref{fig:accuracy:trace_analysis_window:google11:diskIO} show
          %	variations on CPU usage and disk IO time for the Google trace.
        }
\vspace{-0.1in}
\label{fig:accuracy:trace_analysis_window}
\end{figure*}
\fi


\begin{figure*}[tp]
%\vspace{-0.1in}
\centering
\subfigure[Task runtime -- 2Sigma]
{
\includegraphics[width=0.2\linewidth]{figures/trace_analysis/slidingWindow_analysis_unified_cdf_of_covs_in_avg_task_runtime_for_user_name_in_2Sigma_sp3.pdf}	% done
\label{fig:accuracy:trace_analysis_window:sp3:2Sigma:task_dur}
}
\hspace{-12pt}
\subfigure[Task runtime -- Google 11]
{
\includegraphics[width=0.2\linewidth]{figures/trace_analysis/slidingWindow_analysis_unified_cdf_of_covs_in_avg_task_dur_for_application_name_in_google11_sp3.pdf}	% done
\label{fig:accuracy:trace_analysis_window:sp3:google11:task_dur}
}
\hspace{-12pt}
\subfigure[Task runtime -- Google 19]
{
\includegraphics[width=0.2\linewidth]{figures/trace_analysis/slidingWindow_analysis_unified_cdf_of_covs_in_avg_task_dur_for_application_name_in_google19_sp3.pdf}	% done
\label{fig:accuracy:trace_analysis_window:sp3:google19:task_dur}
}
\hspace{-12pt}
\vspace{-0.1in}
\subfigure[CPU usage -- Google 11]
{
\includegraphics[width=0.2\linewidth]{figures/trace_analysis/slidingWindow_analysis_unified_cdf_of_covs_in_mean_CPU_usage_for_application_name_in_google11_sp3.pdf}	% done
\label{fig:accuracy:trace_analysis_window:sp3:google11:cpuUsage}
}
\hspace{-12pt}
\subfigure[Disk IO time -- Google 11]
{
\includegraphics[width=0.2\linewidth]{figures/trace_analysis/slidingWindow_analysis_unified_cdf_of_covs_in_mean_diskIO_time_for_application_name_in_google11_sp3.pdf}	% done
\label{fig:accuracy:trace_analysis_window:sp3:google11:diskIO}
}
\vspace{-0.1in}
\caption{CDF of CoV of runtime properties across space and across time with
	varying history windows, using the 2Sigma, Google 2011 and Google 2019
	traces.  Single-task jobs are excluded from the analysis across space.
        %	This is with 3\% sampling.
}
\vspace{-0.1in}
\label{fig:accuracy:trace_analysis_window:sp3}
\end{figure*}



\if 0
\questionaj{In fig~\ref{fig:accuracy:trace_analysis_window} the sampling
percentage used is 5\%. Earlier we justified 5\% because in our experiments we
used 5\% sampling ratio. However, this is not the case anymore. Now we have an
adaptive sampling based design. The more the sampling percentage the better is
Space CoV, as the formula for Space CoV is inversely proportional to square
root of sampling percentage. So we need to answer this part fairly that why did
we choose 5\% only in this analysis why not 1 or 10.}
\fi

\paragraph{Variation across space.} 
To measure the extent of variation across space, we look at the
CoV (CoV $= \frac{\sigma}{\mu}$) in the task
runtimes within a job.  As shown in \S\ref{sec:accuracy:quantity}, the variance in
the task runtime predicted from sampling is $\frac{\sigmaonesqrd}{m}$, where
$\sigmaonesqrd$ is the variance in the runtimes across all the tasks within the job
and $m$ is the number of tasks sampled.
Thus, we first estimate $\sigma_1^2$ from all tasks within the job. We then report the CoV of our task runtime prediction after sampling $m$ tasks as
%     Thus, the observed \textit{CoV} in the
%     task runtimes within a job after sampling $m$ tasks becomes
$\frac{\sigmaone/\sqrt{m}}{\mu}$.
%= \frac{cov}{\sqrt{m}}$,
%where $\sigmaone$ is the standard deviation in the runtimes of all the tasks of
%the job, $m$ is the number of tasks sampled (5\% of the total tasks) and $\mu$
%is the average task runtime.
Our complete scheduler design in \S\ref{sec:study:design}
uses an adaptive sampling algorithm which mostly uses 3\%
for the three traces.
% Empirically (\S\ref{sec:sim:numPilots}), we found that sampling 5\% of the
% total tasks gives considerably low variation in the predicted tasks runtimes.
Thus, for measuring the extent of variation across space here, we assume
a 3\% sampling ratio and plot
$\frac{\sigmaone}{(\sqrt{0.03\times numberOfTasksInJob}\ )\times\mu}$.

% {We start the analysis on the day after the largest window value
%   so that we can compare the CoVs for the same jobs when varying the history length.
%  }
\paragraph{Variability comparison.}
For consistency, all
analysis results here 
% CDF curves in Fig.~\ref{fig:accuracy:trace_analysis_window:sp3}
are for the same, shortest 
trace period that can be used for sliding-window-history based analysis, \eg the last 15
days under the 14-day window for the 29-day Google 2011 trace.
(The analysis then varies the length of the sliding window in history-based learning.)
%  Fig.~\ref{fig:accuracy:trace_analysis_window:sp3:2Sigma:task_dur}--Fig.~\ref{fig:accuracy:trace_analysis_window:sp3:google19:task_dur} show the CDFs of CoVs
%    the 14-day window for the Google 2011 trace.
  %  However, table
  %  \ref{table:accuracy:trace_analysis:covs:sp3} shows the value for the maximum
  %  possible period.}
\iftoggle{techreport}{ 
Figure~\ref{fig:accuracy:trace_analysis_window:2Sigma:task_dur:scatter}
visualizes the two CoVs for each of 70 randomly selected jobs from the 2Sigma
trace in the order of their arrival, also using the best window size of 14
days.}{}
\rm{For clarity, we first show the result for 70 jobs extracted at
random from the 2Sigma trace, plotted in the order of job arrival in
Figure~\ref{fig:accuracy:trace_analysis_window:2Sigma:task_dur:scatter}.
For each job, we plot the following two values on the y-axis:
%
(1) the CoV in average task runtime for the jobs
in the job's history window, for the feature that gives the least CoV,
using 30-day history window which was found to give the least
variation across history as shown in
Figure\ref{fig:accuracy:trace_analysis_window:2Sigma:task_dur}; and
(2) the CoV in task runtimes of the job.  We see that for both traces, the
variation across history is higher than the variation across tasks for more
than 85\% of the jobs.
}

\iftoggle{techreport}{ 
\begin{figure}[tp]
\vspace{-0.1in}
%\includegraphics[width=1.0\textwidth]{figures/trace_analysis/slidingWindow_analysis_the_scatter_plot_avg_task_dur_in_google11_initial_history_window_3_days.pdf} %done
%\label{fig:accuracy:trace_analysis_window:google11:task_dur:scatter}
%\includegraphics[width=6.5in]{figures/trace_analysis/slidingWindow_analysis_the_scatter_plot_avg_task_runtime_in_2Sigma_initial_history_window_30_days.png} %done
\mbox{\hspace{-0.3in}}\includegraphics[width=1.2\columnwidth]{figures/trace_analysis/slidingWindow_analysis_the_scatter_plot_avg_task_runtime_in_2Sigma_initial_history_window_30_days.pdf} %done
%\label{fig:accuracy:trace_analysis_window:2Sigma:task_dur:scatter}
\vspace{-0.25in}
	\caption{CoVs across time and space
	for 70 jobs selected randomly from the 2Sigma trace.
% 	As evident from Figure
%	\ref{fig:accuracy:trace_analysis_window:2Sigma:task_dur} 30-day history
%	window gives lowest CoVs across time so we choose 30 days as history
        %	period to calculate CoVs across time.
        The x-axis represents job ids in the order of their arrival.}
\vspace{-0.1in}
\label{fig:accuracy:trace_analysis_window:2Sigma:task_dur:scatter}
\end{figure}
}{}


%      The high variability across history can be
%      explained as follows. For the Google trace, more than 67\% of the jobs studied
%      were non-recurring, \ie no exact same job was found for them in history, and
%      only 9\% jobs had more than 20\% of all historical jobs as recurring instances.
%      For this analysis, we
%      follow~\cite{corral, morpheus}, and identify two jobs as recurring instances
%      when they have the same jobname and are being executed by the same application.
%      We did
%      not find recurring jobs in the 2Sigma trace. That is what this statement is
%      saying that we were not able to any such information from the 2 Sigma trace.}
%      The lack of a large number of recurring jobs in the histoy window in turn leads
%      to high error in prediction.



{Fig.~\ref{fig:accuracy:trace_analysis_window:sp3:2Sigma:task_dur}--Fig.~\ref{fig:accuracy:trace_analysis_window:sp3:google19:task_dur}
show the CDFs of CoVs in task duration measured across space and across history
for multiple history window sizes for the three traces.
\if 
{For the 2Sigma (Google 2011) trace, the CoV across history is higher than the
CoV across tasks for 81\% (77\%) of the jobs.  In particular, for more than
30\% of the jobs, the CoV across history is at least 7.13 (26.81) times higher than
the CoV across tasks.  }
\fi
  We see that in general using a shorter sliding window reduces the prediction
  error of 3Sigma, and the CoVs across tasks are moderately lower than the CoVs
  across history for the Google 2011 trace but significantly lower for 2Sigma
  and Google 2019 traces.  For example, for the 2Sigma trace, the CoV across
  history is higher than the CoV across tasks for 85.40\% of the jobs
  (not seen in Fig.~\ref{fig:accuracy:trace_analysis_window:sp3:2Sigma:task_dur}
  as jobs are ordered differently in different CDFs)
  and for
  more than 30\% of the jobs, the CoV across history is at least 12.10$\times$
  higher than the CoV across tasks.
\if 0
{ aj: 2STrace values for 14 days window. 85.40 for gt1 and 12.12 f30 percentile.
Space COVs P50 (P90) 1.00 (3.10)
}
\fi

\if
{For the 2Sigma (Google 2011) [Google 2019] trace, the CoV across history is higher than the
CoV across tasks for 85.68 (71.94) [80.64]\% of the jobs.  In particular, for more than
30\% of the jobs, the CoV across history is at least 12.54 (18.22) [2.89] $\times$ higher than
the CoV across tasks.}
\fi

Table~\ref{table:accuracy:trace_analysis:covs:sp3} summarizes the results,
where the CoVs across time correspond to the best history window size, \ie 3
days for both of the Google traces and 14 days for the 2Sigma trace.  As shown in the table,
% the 50th (90th) percentile CoV, denoted as
the P50 (P90) CoV across
history are 1.00 (3.10) for the 2Sigma trace, 0.20 (0.73) for the Google 2011
trace, and 1.35 (1.67) for the Google 2019 trace.
%
In contrast, the P50 (P90) CoV value across the task duration of the same set
of jobs is much lower, 0.18 (0.55) for the 2Sigma trace and 0.04 (0.58) for the
Google 2011 trace. The P50 (P90) task duration CoV value for the Google 2019
trace, 0.70 (1.33), is higher compared to those of the other two traces, but is
still much lower when compared to the CoV across history for the same trace,
1.35 (1.67).

%\comment{any insights for why?}

%   \commentaj{Yes, I think it could be due to clusterG's high Machine utilization.
%   This means tasks have easy access to resources and hence they do not get
%   swapped in and out and finish within their time. I did some study on this
%   earlier, I am looking into it more today. Additionally, for 2019 trace this is
%   not the case with all the clusters. I looked up for cluster B and cluster H
%   task CoVs. P50 (P90) values for them are 0.09 (0.51) and 0.13 (0.64)
%   respectively. History CoVs for cluster B are 0.39 (2.12)}
%
% {For the 2Sigma (Google) trace, for more than 30\% of the
%   jobs, the CoV across history is at least 10 (35) times higher than the CoV across tasks.
  % for next 20\% it is somewhere between 10-4 (35-15). CoV across history is higher than CoV
% across tasks only for 13\% (16\%) of the jobs.}
%

\rm{The CoV values across tasks is much lower because the tasks of a job run the
same code with the same flags, settings and priority, as mentioned in the trace
schema released by
Google~\cite{googleClusterData2011-2Schema,googleClusterData2019Schema} and
confirmed by 2Sigma engineers~\cite{personalCommunication:MarkAstley}.
% Hence the predictions made by sampling tasks should have a low error.
}

{Fig.~\ref{fig:accuracy:trace_analysis_window:sp3:google11:cpuUsage} and
Fig.~\ref{fig:accuracy:trace_analysis_window:sp3:google11:diskIO} further show the
CDF of CoVs for CPU usage and Disk IO time for the Google 2011 trace (such resource
usage is not available in the 2Sigma trace).
%\addaj{The CoVs here were also measured in the same way as for the task durations.}
%  We use the same
%  methodology for plotting these figures as we did for the task durations.
% We plot in Fig.~\ref{fig:accuracy:trace_analysis_window}
% the variation across space and time for all the jobs in the two traces.
%  For the Google trace, we measure the variation in
%  three runtime properties: Task duration, CPU usage and Disk IO
%  time. In the 2Sigma trace, resource usage is not available and hence
%  we only measured the variation in task duration.
%
The figures show that the variation in the values of these properties when
sampled across space is also considerably lower compared to the variation
observed over time.
}

\if 0
\begin{table}[tp]
%\vspace{-0.05in}
  \caption{CoV in task runtime across time and across space for the
	the 2Sigma, Google 2011, and Google 2019 traces. \commentaj{The 2019 trace values are not correct.}}
\label{table:accuracy:trace_analysis:covs}
\centering
{\small
\vspace{-0.1in}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Trace       & \multicolumn{2}{|c|}{CoV over Time} &
\multicolumn{2}{|c|}{CoV over Space}  \\
\cline{2-5}
			& P50  & P90& P50 & P90 \\
%\hline
\hline
	2Sigma & 0.63 & 2.99 & 0.15 & 0.84 \\
	 %Trace &  & &      &\\
\hline
	Google 2011 & 0.50 & 2.87 & 0.04 & 0.58 \\
	%Trace &    &&&\\
\hline
	Google 2019 & 1.35 & 1.67 & 0.70 & 1.33 \\
	%Trace &    &&&\\
\hline
%\vspace{-0.2in}
\end{tabular}
}
\vspace{-0.1in}
\end{table}
\fi

\begin{table}[tp]
%\vspace{-0.05in}
  \caption{CoV in task runtime across time and across space for the
    the 2Sigma, Google 2011, and Google 2019 traces.
    % with 3\% sampling.
    %    \commentaj{the 2019 trace values are not correct.}
  }
\label{table:accuracy:trace_analysis:covs:sp3}
\centering
{\small
\vspace{-0.1in}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Trace       & \multicolumn{2}{|c|}{CoV over Time} &\multicolumn{2}{|c|}{CoV over Space}  \\
            \cline{2-5}
			& P50  & P90& P50 & P90 \\
%\hline
\hline
	%2Sigma & 0.63 & 2.99 & 0.12 & 0.65 \\
	2Sigma & 1.00 & 3.10 & 0.18 & 0.55 \\
	 %Trace &  & &      &\\
\hline
	%Google 2011 & 0.50 & 2.87 & 0.03 & 0.45 \\
	Google 2011 & 0.20 & 0.73 & 0.04 & 0.58 \\
	%Trace &    &&&\\
\hline
	Google 2019 & 1.35 & 1.67 & 0.70 & 1.33 \\
	%Trace &    &&&\\
\hline
%\vspace{-0.2in}
\end{tabular}
}
\vspace{-0.2in}
\end{table}


\subsection{Experimental Prediction Error Analysis}
\label{sec:accuracy:experiment}

\if 0
To validate the analysis from \S\ref{sec:accuracy:quantity} 
that lower task-wise variation than job-wise
variation (\S\ref{sec:accuracy:trace}) will translate into better
prediction accuracy of sampling-based schemes over history-based
schemes, we next implement a sampling-based predictor \slearn and
experimentally compare it against a state-of-the-art history-based
predictor \primarybasepredict~\cite{3Sigma} in estimating the job
runtimes.
\fi

Recall from our analysis in \S\ref{sec:accuracy:quantity}
that lower task-wise variation than
job-wise variation (\S\ref{sec:accuracy:trace}) will translate into better prediction
accuracy of sampling-based schemes over history-based schemes. While
our analysis in \S\ref{sec:accuracy:quantity}
assumes normal distribution, we believe that a
similar conclusion will hold in more general settings. To validate
this, we next implement a sampling-based predictor \slearn,
and experimentally compare it against a
state-of-the-art history-based predictor 3Sigma~\cite{3Sigma} in estimating the
job runtimes directly on production job traces.

%The experimental setup used for this comparison is described below.
\paragraph{Workload characteristics.}
{Since the three production traces described in
\S\ref{sec:accuracy:trace} are too large,
as in 3Sigma~\cite{3Sigma},
we extracted smaller traces for experiments
% We extracted roughly 1250 jobs each from the three production traces
using the procedure described below.
%  We denote the traces extracted
% from 2Sigma~\cite{2Sigma:trace}, Google 2011 version~\cite{googleTraceGithub}
% and Google 2019 version~\cite{googleClusterData2019}
% These extracted jobs form the traces that we will experiment with,
We denote the extracted traces which consist of roughly 1250 jobs each
as 2STrace, GTrace11 and GTrace19, respectively.

Since the history-based predictor 3Sigma needs a history trace,
we followed the same process as in~\cite{3Sigma} to extract the training
trace for 3Sigma and the execution trace for all predictors, in three steps.
(1) We divided each original trace in chronological
order in two halves.
(2) We next selected the execution trace following the process below
from the second half; these became 2STrace, GTrace11 and GTrace19,
respectively.
(3) We then selected jobs from the first half of each original trace
that are feature-clustered with those jobs in the execution trace to form
the "history" trace for 3Sigma.

We extracted the execution trace from the above-mentioned second halves as follows.
  % Since the 2Sigma trace has many wide jobs that are wider than the number
In extracting 2STrace,
since the original cluster from where the 2Sigma trace was collected 
(441 nodes, each with 24 cores) is much larger than
our experimental cluster (150 single-core nodes),
we resized the job widths to preserve
the job-width-to-cluster-size ratio by randomly dropping tasks
%   In particular, 
%   we randomly dropped some tasks from each
%   job so that the ratio of each job's width 
%   to the size of our 150-node clusetr remains the same as its job width
%   in the original 2Sigma trace to the orignal cluster size,
and then randomly selected 1250 jobs with equal probability as the 2STrace.
\if 0
Since the original 2Sigma trace does not specify
how many cores were used by each job task,
we assumed that each task uses 1 core, same as in \primarybasepredict~\cite{3Sigma}.
With this assumption,
we calculated the effective number of cores per machine to be 5.49 in
order for the average workload of the original trace to remain 1.0
(This ensures no persistent queue build-up in the cluster).  Using
this effective cluster size, we randomly dropped some tasks from each
job so that the ratio of job width 
to cluster size in 2STrace on our 150-node cluster remains the same as
in the original 2Sigma trace then randomly uniformly selected 1250 jobs from
the remaining jobs as the 2STrace.
\fi
}
\if 0
To extract GTrace11 and GTrace19,
  % we followed the following process.
  % Based on a suggestion from a Google engineer,
we first dropped single-task jobs from both Google traces for two
  reasons following~\cite{personalCommunication:Nan}: (1) these jobs make less
  than 1\% of the total workload, (2) most of these jobs are test jobs
  and their performance are considered as not important.
  %
  Next,
\fi
%
Similarly, since the Google traces do not have many wide jobs yet the
original clusters are very wide, with ~12.5K machines, we dropped jobs
with more than 150 tasks, and randomly selected 1250 jobs with equal
probability from the remaining jobs to create GTrace11 ad GTrace19,
respectively.  

  \if 0
  Another reason to choose the
  \textit{clusterG} from 2019 trace is that, as shown in the trace
  analysis paper~\cite{borgTraceAnalysis2019}, it has highest machine
  utilization and the 2011 trace has machine utilization lower than
  any of the clusters in 2019.
  \fi

Finally, for each extracted trace, we adjust the arrival time of the
jobs so that the average cluster load matches that in the original
trace~\cite{2Sigma:trace,googleTraceGithub,googleClusterData2019}.
Table~\ref{table:accuracy:load:stats} summarizes the workload
per window of the extracted traces, where a window is defined
as a 1000-second interval sliding by 100 seconds at a time,
and the load per window is the total runtime of all the jobs arrived in that window,
normalized by the total number of CPUs in the cluster times the window length, \ie 1000s.
We see that for all three traces, the average system load is close to 1, though 
the load fluctuates over time, which is preserved by the random uniform job extraction.

\begin{table}[tp]
  \caption{Statistics for system load per 1000s sliding window.}
  \label{table:accuracy:load:stats}
  \vspace{-0.1in}
  \centering
      {
\small
\begin{tabular}{|c|c|c|c|c|c|}
\hline
		 Trace       & Average &  P50 & P90\\
%\hline
\hline
	2STrace & 1.05  & 0.13 & 2.47 \\
\hline
	GTrace11 & 1.01  & 0.29 & 1.49 \\
\hline
	GTrace19 & 1.04  & 0.09 & 0.91 \\
\hline
\end{tabular}
}
  \vspace{-0.1in}
%  \vspace{-0.2in}	% AJ_spacecut
\end{table}

%\addaj{Finally, for each extracted trace, we appropriately compressed the arrival time
%of the jobs so that the average cluster load remains 1.0, which we assumed is
%the case in the orignal trace as otherwise there would be persistent job queue
%build-up.}

% \addaj{\textbf{Pretraining history based predictors:} Since the experimental traces
% are only 1250 jobs, the history based predictors needs to be pretrained.

\if 0
\paragraph{Workload characteristics.}
{Starting with the two production cluster traces described in
  \S\ref{sec:accuracy:trace}, we filtered out jobs with more than 150
  tasks since our cluster size is 150 nodes.
Following 3Sigma~\cite{3Sigma}, we extracted 1250 jobs from full traces for simulation
and testbed experiments in order to expedite the experiments.
% 
We then extracted two test traces, GTrace and 2STrace, each having
1250 jobs randomly selected from the corresponding filtered
traces. The traces are xx and xx hours long respectively.  For
both of them, we maintain the job arrival time distribution similarly
as in the original traces.  We then extracted corresponding training
data for the history-based predictor \primarybasepredict, which
contains 3,000 jobs each randomly selected from the filtered traces,
using the correspondingly best history windows observed in
\S\ref{sec:accuracy:trace}.
\commentaj{write about trace width compression here.}
\addaj{Write following points: We removed all the single task jobs from the
experimental traces as single task jobs make a very insignificant (less than
0.5\%) portion of the total runtime and resource usage. Same thing was confirmed
to us in a personal conversation by a Google engineer that they don't care much
about single task job. Also, in many cases job masters are run as a separate
single-task job.}
\rm{We assume each task in the trace requires one node and zero memory.}
\fi


\if 0 
To measure the accuracy of \lTechnique or \primarybasepredict
on the extracted job traces,
we simulated a generic job scheduler on a cluster of 150 nodes
that minimizes the average job completion time by using
job runtime estimated by either \lTechnique or \primarybasepredict,
while replaying each job trace.
The detailed experimental setup is described in \S\ref{sec:study:design}.
%  Since the goal of this experiment is to
%  compare the prediction accuracy, which is independent of the scheduling mechanism.
%  we skip the scheduling details here.   
\fi

\if 0
    {We need to discuss this. What should we do regarding the sampling
percentage in \S\ref{sec:accuracy:trace} and \S\ref{sec:accuracy:experiment}.
The current value used for figure~\ref{fig:accuracy:trace_analysis_window} and
\ref{fig:accuracy:trace_analysis_window:2Sigma:task_dur:scatter} is 5\%. The
values in figure~\ref{fig:sim:estimationAccuracy} are for the adaptive
sampling.}
    \fi

    
\paragraph{Prediction mechanisms and experimental setups.}
%\label{subsec:setup}
We implement the \primarybasepredict predictor following its description in~\cite{3Sigma}.
After learning the job runtime distribution (\S\ref{sec:accuracy:trace}),
it uses a utility function of the estimated job runtime
associated with every job to derive its estimated runtime from the
distribution, by integrating the utility function
over the entire runtime distribution.
Since our goal is to minimize the average JCT, we used a utility function that is inversely
proportional to the square of runtime. 
% To ensure correct execution of \primarybasepredict,
We kept all the default settings
% in a private communication~\cite{personalCommunication:JunWoo} with
we learned from the authors of 3Sigma~\cite{3Sigma}.
% and kept all the settings and parameters in our implementation the same 
% as in 3Sigma~\cite{3Sigma}.

As in \S\ref{sec:accuracy:trace}, \slearn
samples
% the number of sampled tasks assigned to a job in \lTechnique is
$max(1, 0.03 \cdot S)$ tasks per job, where $S$ is the number of tasks in the job.
%  We used 5\% sampling fraction to keep the experimental analysis
% the same as the trace analysis
% (\S\ref{sec:accuracy:trace}).
{We only show the results for wide jobs (with \thinLimit or more
  tasks) as in the complete \slearn design (\S\ref{sec:design:gs}),
  only wide jobs go through the sampling phase.  }


%\begin{figure*}[tp]
%\centering
%\subfigure[2STrace]
%{
%\includegraphics[width=0.33\linewidth]{figures/simulation/prediction_error_new_2STrace.pdf}
%%\caption{Job runtime learning accuracy for the 2Sigma trace.}
%\label{fig:sim:estimationAccuracy:2STrace}
%}
%\hspace{-0.25in}
%\subfigure[GTrace11]
%{
%\includegraphics[width=0.33\linewidth]{figures/simulation/prediction_error_new_GTrace11.pdf}
%\label{fig:sim:estimationAccuracy:GTrace11}
%}
%\hspace{-0.25in}
%\subfigure[GTrace19]
%{
%\includegraphics[width=0.33\linewidth]{figures/simulation/prediction_error_new_GTrace19.pdf}
%\label{fig:sim:estimationAccuracy:GTrace19}
%}
%\vspace{-0.15in}
%	\caption{Job runtime prediction accuracy \updated{all - 16th Sep 2020}}
%\vspace{-0.15in}
%\label{fig:sim:estimationAccuracy}
%\end{figure*}

\begin{figure*}[tp]
\centering
\subfigure[2STrace]
{
\includegraphics[width=0.32\linewidth]{figures/simulation/offlinePredictionError_2STrace_sp3.pdf}
\label{fig:sim:estimationAccuracy:2STrace}
}
%\hspace{-0.25in}
\subfigure[GTrace11]
{
\includegraphics[width=0.32\linewidth]{figures/simulation/offlinePredictionError_GTrace11_sp3.pdf}
\label{fig:sim:estimationAccuracy:GTrace11}
}
%\hspace{-0.25in}
\subfigure[GTrace19]
{
\includegraphics[width=0.32\linewidth]{figures/simulation/offlinePredictionError_GTrace19_sp3.pdf}
\label{fig:sim:estimationAccuracy:GTrace19}
}
\vspace{-0.15in}
\caption{Job runtime prediction accuracy.
  % For \slearn we assumed the sampling ratio to be 3\%. \updated{all - 25th Sep 2020}
}
\vspace{-0.15in}
\label{fig:sim:estimationAccuracy}
\end{figure*}

\paragraph{Results.}
Fig.~\ref{fig:sim:estimationAccuracy} shows the CDF of percentage error in the predicted
job runtimes for the three traces.
% where error = $\frac{abs(predicted\_dur\ -\ actual\_dur)}{actual\_dur}\times100$.
{We see that \slearn has much better prediction accuracy than
  \primarybasepredict.} For 2STrace,
GTrace11, and GTrace19,
the P50 prediction error
are 18.30\%, 9.15\%, 21.39\% for \namepredict
but 36.57\%, 21.39\%, 71.56\% for \primarybasepredict, respectively,
and the P90 prediction error
% for 2STrace, GTrace11, and GTrace19
are 58.66\%, 49.95\%, 92.25\% for \namepredict
but 475.78\%, 294.52\%, 1927.51\% for \primarybasepredict, respectively.

\if 0
For 2STrace, the P50 (P90) estimation error is 
		18.98\% (62.38\%) for \slearn and
        36.57\% (475.78\%) for \primarybasepredict.
        For GTrace11, the estimation error is  13.67\% (59.92\%)
        for \slearn and 24.52\% (294.52\%) for \primarybasepredict.
        For GTrace19, the estimation error is  51.84\% (94.43\%)
        for \slearn and 71.56\% (1927.51\%) for \primarybasepredict
\fi

        
\if 0
\commentaj{Cluster G from 2019 has very high error. However, that is not the
case with all the cluster of 2019. I tried with other cluster H with all tier
jobs. That also has a speed up 1.25$\times$ and P50 (P90) error for \slearn is
1.23 (9.39)\% and for \primarybasepredict it is 8.63 (53.60)\%. With cluster B
beb-tier jobs the speedup is 1.9$\times$ and P50 (P90) error for \slearn is
7.65 (58.68)\% and for \primarybasepredict it is 28.72 (144.01)\%. I think we
can use this result somewhere as clusterG 2019 has very high error for both
\slearn and \primarybasepredict.}
\fi

\if 0
{The average prediction error for 2STrace (GTrace) is 27.46 (19.24)\% for \namepredict
but 552.03 (81.35)\%} for \primarybasepredict.
\fi
%  These results
%  show that a sampling-based predictor can predict with better accuracy than the
%  state-of-the-art history-based predictor.

% These results support the conclusion of the quantitative and the trace analysis. 

We observe that the predictor error for GTrace19 is higher than
that for 2STrace and GTrace11
% which in turn is higher than forGTrace11
when we use either history-based or sampling-based prediction.  This is because 
GTrace19 has higher CoV values for the average task runtimes, both across the
history and across the tasks of the same job
(Table~\ref{table:accuracy:trace_analysis:covs:sp3}). This result also confirms
that the prediction accuracy of both schemes are directly affected by the
variance (\S\ref{sec:accuracy:quantity}).
% {GTrace19 has the highest prediction errors, though we could not analyze its job CoV values due to lack of job information (\S\ref{sec:accuracy:trace}).}
%   GTrace19 has relatively high prediction errors, which is explained by its
%   high CoV values across both spacce and time as discussed in
%   \S\ref{sec:accuracy:trace}.


\if 0
    {To measure the impact of \primarybasepredict's high estimation error in
a job scheduling algorithm, \eg SJF, 
  %  we measured the chances of pairwise order of wide jobs getting
  % swapped from their actual order. \ie
we sorted the jobs in the increasing order of their sizes, and measured how often
the order of each pair of jobs becomes flipped due to incorrect job size
estimation error.  Table~\ref{table:accuracy:trace_analysis:fliprate} shows the
results.  We observe that for the 2STrace, GTrace11, and GTrace19, 23.71\%,
25.83\%, and 39.72\% of job pairs are flipped by \primarybasepredict whereas
only 8.58\%, 13.03\%, and 18.03\% are flipped by \name, respectively.

%  . \ie when runtimesare predicted using \name the chance that the jobs will be sorted in correct
%  order is 94.13\% (91.00\%) for the 2Sigma (Google) trace whereas when
%  \primarybasepredict is used the chances fall down to 78.77\% (76.99\%). If job
%  pairs are to be ordered randomly the chance of correct ordering will be 50\%.
%the chances of flipping are $3.62 \times$ $(2.15 \times)$ higher for the
%\primarybasepredict as compared to the \namepredict


\begin{table}[tp]
%\vspace{-0.05in}
  \caption{Chances of correctly ordering pairs of jobs
    for all unique job pairs in each trace.
    %  . We have counted unique pairs. \commentaj{If we show the number of pairs which can flip then it is 2 times for google traces and 3 times for 2 Sigma.} \updated{all - 16th Sep 2020}
  }
\label{table:accuracy:trace_analysis:fliprate}
\centering
{\small
\vspace{-0.1in}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
		 Trace       & \name &  \primarybasepredict & Random\\
			& (Space)  &  (Time) & (No info) \\
%\hline
\hline
	2STrace & 91.42\%  & 76.29\% & 50.00\% \\
\hline
	GTrace11 & 86.97\%  & 74.17\% & 50.00\% \\
\hline
	GTrace19 & 81.97\%  & 60.28\% & 50.00\% \\
\hline
%\vspace{-0.2in}
\end{tabular}
}
\vspace{-0.1in}
\end{table}
\fi


\if 0
In summary, our quantitative, trace-based and experimental analysis
have shown that a sampling-based scheme can predict job runtime
characteristics with considerably higher accuracy than
a state-of-the-art history-based predictor.
\fi


==> deadline-design.tex <==
\paragraph{Learning for deadline jobs.}
\label{sec:discuss:maxTaskLength}
%
In multi-tenant job clusters, different jobs may have different 
SLOs. 
% To evaluate the effectiveness of sampling on other types of scheduling goals, 
We performed an initial study of the effectiveness of a sampling-based scheme
% developed another scheduler \gsdl from \gs 
% to minimize deadline misses. 
to predict the max task length for use by a deadline scheduler
to minimize deadline misses (\eg~\cite{jockey:eurosys2012}).
In particular, we revised both \slearn and \primarybasepredict to 
predict the maximum task length using
the maximum observed task length from sampling and history respectively.
%
\if 0
\gsdl's architecture is similar to that of \gs and differ in two ways:
(1) The sampling-based predictor is tuned to predict
the maximum task length, since for a job to finish within deadline, it is
required that the longest task finishes within the deadline. 
\comment{Accordingly, \slearn now estimates the maximum task length as the length
of the longest running sampled task. Similarly, the history-based predictor
estimates the maximum task length by ????
} (2) \gsdl schedules jobs with estimated max task lengths by ???
\fi
%
{
Figure~\ref{fig:sim:estimationAccuracy-max} shows the CDF of
estimation error of maximum task length (normalized by the true max
task length) for the two traces. We see that for GTrace
the mean prediction error is 31.17\% for
\slearn but 116.51\% for \primarybasepredict
though the errors are comparable for 2STrace.  One nice feature
about \slearn is that its error is upper-bounded by 100\% while the
error of \primarybasepredict can go unbounded.
}
%  is similar between \slearn and \primarybasepredict, and thus
%  sampling appears to have no added benefit over history-based prediction 
%  in predicting the max value of job properties.
Motivated by 
this preliminary result, and because deadline scheduling typically require both the
max task length and the total resource requirement of the jobs~\cite{morpheus,3Sigma}
%   Previous work has shown that tasks from the same stage have
%  similar resource requirements~\cite{pacman:nsdi12, drf:nsdi11,
%  paratimer:sigmod2010}.  
and the later can be more accurately estimated by sampling, we plan to
explore sampling-based prediction for deadline scheduling in our
future work.

\if 0
As we can estimate the total resource
requirement by estimating the average resource requirement by sampling
a few tasks.\\ Our case study I (\S\ref{sec:study}) and analysis
in \S\ref{sec:accuracy} have shown that sampling is significantly
better than a history based approach for predicting an average of a
property.
\fi


\if 0
\deadlineCS{To evaluate the impact of sampling on another class of scheduling
goals like SLO misses, we did another study. We deriverd another scheduler
\gsdl from \gs. \gsdl's architecture is same as \gs and we also kept the
default settings same. \gsdl differs \gs only in following two ways: (1)
\textbf{No multiple priority queue in \gsdl}: Unlike \gs, \gsdl doesn't need a
starvation freedom mechanism, as the jobs which miss deadline are dropped.
Hence all the jobs are kept in a single queue called as main queue.  However,
other than the main queue \slearn uses two more queues, one for sampling and
another for thin jobs.  (2) Jobs in the main queue are sorted on the basis of
the $slack$ a job has from its deadline, where $slack = deadline - (arrivalTime
+ estimatedJobDuration)$. Jobs with negative $slack$ are not admitted.\\
\paragraph{Predictors:} Like \gs, different predictors can be plugged into
\gsdl. However, in this study predictors are tuned to predict maximum task
length.  Since for a job to finish within it is required to ensure that the
longest task finishes within the deadline. Therefore, training data for the
distribution based predictor, 3Sigma, and the point estimate predictor consists
maximum task length. \slearn uses the maximum task length observed from all the
sampled tasks.\\ 
Additionally, leveraging the above observation \gsdl drops a job if it has
even one unscheduled task at $t = deadline - jobDuration$ time.\\
\paragraph{Workloads:} We used the same set of workloads, GTrace and 2STrace,
as used in study I \S\ref{sec:study}. The original Google trace and 2Sigma
trace do not have deadline information. We derived deadlines keeping consitency
with the obeservations made in previous works like Morpheus~\cite{morpheus} and
Tetrisched~\cite{tetrisched}. Also, we stretched job inter-arrival time such
that with a fully accurate predictor \gsdl can finish more than 90\% jobs
within deadline. For each job we set the deadline to be $t \times
maxTaskLength$ from its arrival time. We varied $t$ from 2.6 to 3.4 with a step
of 0.2.\\
\paragraph{Results:} We have summarized the job drop rate for \slearn and
\primarybasepredict in the table~\ref{table:study2:jobsDropped:2STrace} for the
2STrace and in table~\ref{table:study2:jobsDropped:GTrace} for the GTrace.  
\begin{table}
  \caption{Number of jobs dropped for 2STrace}
\label{table:study2:jobsDropped:2STrace}
  \centering
      {\small
	\begin{tabular}{|c|c|c|c|c|c|}
	  \hline
		Deadline Multiplier&2.6& 2.8&3.0&3.2&3.4\\
	  \hline
		\slearn&910&915&921&925&929\\
	  \hline
		\primarybasepredict &867&881&883&891&895\\
	  \hline
		Point Prediction &866&878&884&891&898\\
	  \hline
		Zero Error &918&919&927&932&935\\
	  \hline
	\end{tabular}
      }
\vspace{-0.1in}
\end{table}
\begin{table}
  \caption{Number of jobs dropped for GTrace}
\label{table:study2:jobsDropped:GTrace}
  \centering
      {\small
	\begin{tabular}{|c|c|c|c|c|c|} 
	  \hline
		Deadline Multiplier&2.6& 2.8&3.0&3.2&3.4\\  
	  \hline
		\slearn&1&2&3&4&5\\
	  \hline
		\primarybasepredict &1&2&3&4&5\\
	  \hline
	\end{tabular}
      }
\vspace{-0.1in}
\end{table}
}
\fi



==> intro-runtimes.tex <==
\section{Introduction}
\label{sec:intro}

\commentaj{This section is written assuming that paper's key point was around
the scheduler. It needs to be updated according to the new outline.}


Use of shared clusters is increasing and clusters have to support diverse set
of activities like including but not limited to data analytics, consumer
services and development services. This is increasing challange for cluster
schedulers to effciently pack jobs and make best use of available resources.

Works like \cite{tetrisched, morpheus, 3Sigma,
Socc14:IfYouAreLateDon'tBlameUs} have shown that having prior knowledge of job
runtimes can help cluster schedulers in making better and more robust
scheduling decisions. However, in most cases runtime estimates are derived
using some form of runtime history of similar jobs. Where notion of similarity
could be based on one or more of the following, job executed by same user, jobs
of same application, jobs demanding similar resource or jobs executed at
similar point in time cycle etc \cite{jamiasvu, 3Sigma}. 

\questionaj{Here, I also want to state that using task runtimes is a
better idea as compared to job runtimes. Because job runtime is difference
between endtime of last task and starting time of first task which also depends
on extent of parallel resource available. However, average task runtime is
independent of that. What do you think?}

If the estimates are accurate scheduler using such prediction mechanism will
provide better results than schedulers those are not. However, using two
production cluster traces we observed that runtimes are long tailed
\todoaj{plot cdf of average runtime figure.} and average task length based on several
classifying features used in \cite{3Sigma} and \cite{jamiasvu} show high degree
of variability \todoaj{plot figures of cov in avg task runtime for features for
the traces.}. Also as shown in \cite{3Sigma} that state-of-the-art job runtime
predictors can have more than 50\% estimation error for 23\% of jobs and in
some cases more than 20\% jobs have extremely high error \questionaj{in 3 sigma
they have show this as tail error and have not written exact numbers, I am not
sure how to write this better.}

\questionaj{how to write here smoothly about job runtimes and average task
length. Values in previous papers are about job runtimes and we should show
average task runtime as we are using average task runtime everywhere. Please
advise.}

Another limitation of using history based predictor is that history gets
outdated due to various reasons like software updates, hardware updates, change
in user demand pattern and number of users.

To overcome the above mentioned challenges In this paper, we propose
\namepredict, a dramatically different approach for online runtime  prediction
for distributed jobs.  And we present \name a complete cluster scheduler which
approximates SJF using \namepredict as it's primary source of runtime
estimates.  For optimal scheduling using SJF in cluster scheduling, it is vital
to learn the task runtimes quickly and accurately. \namepredict achieves this
objective by exploiting the \textit{spatial dimension} of distributed jobs, \ie
a jobs typically consists of many tasks, and by using \textit{sampling}, a
highly effective technique used in large-scale
surveys~\cite{samplingOfPopulations}.  In particular, \namepredict
pre-schedules sampled tasks, called {\em pilot tasks}, of each jobs and uses
their measured runtimes to estimate the average task runtime or job runtime. It
then resorts to SJF using the estimated job runtime.

Scheduling pilot tasks first before the rest of the tasks can potentially incur
two overheads.  First, scheduling pilot tasks of a newly arriving job consumes
resources which can delay other jobs (with already estimated runtimes). To
tackle this \name creates separate logical partitions of cluster and
prioritizes scheduling of tasks of job whose runtime has been estimated on one
and prioritizes scheduling on sampling tasks on other. Size of these partitions
are dynamically adjusted based on queue length. 

Second, scheduling pilot tasks first may elongate the JCT of the newly
arriving job itself whose other tasks cannot start until the pilot
tasks finish. This is again typically insignificant for following reason:
job scheduling is of high relevance in a busy
cluster (when there is a backlog of jobs in the system), in which
case the JCT of job is expected to be much higher than if it were
the only job in the system, and hence the piloting overhead is
further dwarfed by a job's actual JCT.

We present the complete \name design that addresses two major design issues:
%(1) How to schedule the pilot tasks?
(1) How to integrate \namepredict with a cluster scheduler?
(2) How to schedule among all the jobs with estimated runtimes?

We have implemented and evaluated \name using a prototype on a 150-node cluster
in Microsoft Azure, and large-scale simulations {utilizing a public cluster
trace from Google and a private trace from 2Sigma cluster.  Our simulation
results show that, compared to prior art 3Sigma, \name reduces the average JCT
by 1.66$\times$ (1.88$\times$) for Google trace(2Sigma trace) We also evaluated
\name on a testbed.  Our testbed evaluation shows that \name reduces the
average job completion time by 60\% compared to 3Sigma.


In summary, this paper makes the following contributions:
\begin{itemize} %% [noitemsep,topsep=0pt,leftmargin=0.2in]
\item Using two production cluster trace from Google and 2Sigma, we show that
	history might not be a very good predictor for runtime characterstics of a distributed jobs. 
\item We propose, \lTechnique, a novel learning approach for distributed jobs. \lTechnique uses sampling in the spatial dimension
%\item We propose, \namepredict, the novel idea of applying sampling in the spatial dimension
of job to learn job runtime propeties online with very high accuracy.
\item We present the complete design and implementation of \name, a
	\lTechnique based cluster scheduler whose primary goal is to minimize average JCT.
\item We extensively evaluate \name via simulations and testbed experiments,
	and show that compared to the prior art, the new design reduces the
	average JCT by 1.66$\times$ (1.88$\times$) for the Google trace (2Sigma trace).
\end{itemize}


==> old-text.tex <==
%%%% Below from simulation.tex on Sep 16 2020 %%%%
\begin{table}[tp]
	\centering
\caption{Performance improvement of \slearn over \primarybase when the number of pilot
  tasks is varied.
  % {Percentile average task waiting times are calculated after removing thin jobs.}
}
\label{table:sim:numPilots:2STrace}
\vspace{-0.25in}
{\small	
	%\begin{tabular}{cccccccc}
		%\begin{tabular}{cp{0.18in}|p{0.18in}|p{0.18in}|p{0.18in}|p{0.18in}|p{0.18in}|p{0.18in}}
		\begin{tabular}{cp{0.18in}p{0.18in}p{0.18in}p{0.18in}p{0.18in}p{0.18in}p{0.18in}}
		\\ 
% \Xhline{3\arrayrulewidth}
\hline
			 & \multicolumn{7}{c}{Fraction of tasks chosen as pilot tasks}\\
		 &1\%&2\%&5\%&10\%&15\%&20\%&25\%\\  
			    	%Avg. error &X.XXx\%&6.14\%&5.42\%&4.94\%&5.53\%&4.25\%&4.15\%&2.9\%                                    \\
\hline
			& \multicolumn{7}{c}{2STrace \updated{2S - 12th May 2020}}\\
\hline
		     	%P50 pred. error \hspace{-0.1in}&19.01\%&18.23\%&14.04\%&11.80\%&10.94\%&9.46\%&8.39\%                                    \\
			%Avg. JCT speedup \hspace{-0.1in}&1.14&1.14&1.44x&1.38x&1.29x&1.23x&1.17x \\
			%P50 speedup\hspace{-0.1in}&1.28&1.29&1.44x&1.36x&1.31x&1.28x&1.21x  \\
			P50 pred. error (\%) \hspace{-0.1in}&19.35&18.98&18.45&16.95&15.23&14.22&13.32\\
			Avg. JCT speedup ($\times$)\hspace{-0.1in}&1.24&1.23&1.27&1.28&1.21&1.15&1.08  \\
			P50 speedup ($\times$)\hspace{-0.1in}&0.92&0.92&0.94&0.95&0.90&0.84&0.79\\
	      		
			%Avg. job waiting time (KSec) &3882.04&4050.95&4450.96&4524.77&4791.99                                    \\
	      		%P50 avg. waiting time (KSec) &4.66&4.31&4.78&5.41&7.33                                    \\
	      		%P70 avg. waiting time (KSec) &79.02&91.62&107.55&151.72&201.46                                    \\
	      		%P90 avg. waiting time (KSec) &340.62&329.98&315.87&309.55&299.73                                    \\
			
\hline
			& \multicolumn{7}{c}{GTrace \updated{G11 - 9th July 2020}}\\
\hline
		P50 pred. error (\%)\hspace{-0.1in}&10.17&10.09&8.33&5.28&5.35&4.80&4.09\\
		Avg. JCT speedup ($\times$)\hspace{-0.1in}&1.41&1.40&1.43&1.13&0.90&0.76&0.63\\
		P50 speedup ($\times$)\hspace{-0.1in}&1.12&1.12&1.10&1.07&1.02&1.0&0.94\\
		%P50 pred. error \hspace{-0.1in}&8.90\%&8.56\%&7.85\%&6.09\%&4.88\%&4.27\%&3.56\%                                    \\
		%Avg. JCT speedup \hspace{-0.1in}&1.34&1.30&1.40x&1.36x&0.98x&0.84x&0.72x  \\
		%P50 speedup\hspace{-0.1in}&0.86&0.87&0.74x&0.70x&0.73x&0.68x&0.73x \\
\hline
			& \multicolumn{7}{c}{GTrace19 \updated{G19 - 26th Aug 2020}}\\
\hline
		P50 pred. error (\%)\hspace{-0.1in}&56.44&55.64&48.35&43.15&39.39&37.08&33.54\\
		Avg. JCT speedup ($\times$)\hspace{-0.1in}&1.24&1.23&1.18&1.10&0.99&0.92&0.84\\
		P50 speedup ($\times$)\hspace{-0.1in}&1.46&1.30&1.06&0.97&0.84&0.81&0.73\\
\hline
	\end{tabular}
}
\vspace{-0.1in}
\end{table}






\if 0
\begin{table}
\caption{Fraction of overestimated jobs and incorrect queue placement for 2STrace. Job performance in the third column is relative to the \oracle. \updated{2S - 14th June 2020}}
  \label{table:sim:overestimatedJobs}
\vspace{-0.1in}	
  \centering
      {\small
	\begin{tabular}{|c|c|c|c|c|} 
	  \hline
		& Overestima- & Misplaced over- & Slowed misp- & Average (P50)\\
		& ted jobs & estimated jobs & laced jobs & Positive error\\
	  \hline
		%\primarybase & 59.37\% & 36.02\% & 82.84\% \\
		\primarybase & 59.37\% & 21.09\% & 17.72\% & 1253.60 (66.38)\% \\
	  \hline
	  	%\slearn & 43.75\% & 8.09 \% & 100\% \\
	  	\slearn & 43.75\% & 2.87 \% & 2.63\% & 29.64 (17.79)\% \\
	  \hline
	\end{tabular}
      }
\vspace{-0.1in}	
\end{table}

\begin{table}
\caption{Fraction of underestimated jobs and incorrect queue placement for 2STrace. Job performance in the third column is relative to the \oracle. \updated{2S - 14th June 2020}}
  \label{table:sim:underestimatedJobs}
\vspace{-0.1in}	
  \centering
      {\small
	\begin{tabular}{|c|c|c|c|c|} 
	  \hline
		& Underestim- & Misplaced under & Spedup misp- & Average (P50)\\
		& ated jobs & estimated jobs & laced jobs & Negative error\\
	  \hline
		%\primarybase & 40.63\% & 25.15\% & 82.81\% \\
		\primarybase & 40.63\% & 10.22\% & 8.46\% & -39.33 (-31.59)\%\\
	  \hline
	  	%\slearn & 55.45\% & 12.77 \% & 45.83\% \\
	  	\slearn & 55.45\% & 5.75 \% & 2.63\% & -26.13 (-19.61)\% \\
	  \hline
	\end{tabular}
      }
\vspace{-0.1in}	
\end{table}
\fi


%%%% Above from simulation.tex on Sep 16 2020 %%%%



%%%% Below from simulation.tex on Sep 17 2020 %%%%
\if 0
\begin{table*}[tp]
	\centering
\caption{Performance improvement of \slearn over \primarybase for GTrace when the number of pilot
  tasks is varied.
  % {Percentile average task waiting times are calculated after removing thin jobs.}
}
\label{table:sim:numPilots:GTrace}
\vspace{-0.25in}
{\small	
	\begin{tabular}{cccccccc}
		%\caption{GTrace}
		\\ \Xhline{3\arrayrulewidth}
			 & \multicolumn{7}{c}{Fraction of tasks chosen as pilot tasks}      \\
		&1\%&2\%&5\%&10\%&15\%&20\%&25\%	\\  \Xhline{3\arrayrulewidth}
		P50 pred. error \hspace{-0.1in}&8.90\%&8.56\%&7.85\%&6.09\%&4.88\%&4.27\%&3.56\%                                    \\
		Avg. JCT speedup \hspace{-0.1in}&1.34&1.30&1.40x&1.36x&0.98x&0.84x&0.72x  \\
		P50 speedup\hspace{-0.1in}&0.86&0.87&0.74x&0.70x&0.73x&0.68x&0.73x \\
\hline
	\end{tabular}
}
\vspace{-0.1in}
\end{table*}
\fi


%  The two test traces have 1000 jobs each, are 2.25 and 2.15 hours long,
%  respectively, and retain the same job arrival time distribution
%  as the original traces.


\if 0
\begin{figure*}[tp]
\centering
	\subfigure[CDF of normalized task waiting times for all wide jobs]{
	\includegraphics[width=0.31\textwidth]{figures/simulation/normalized_average_task_waiting_time_2STrace.pdf}
	\label{fig:sim:waitingTimesTrial:2STrace:cdf}
	\vspace{-0.1in}
}
	\subfigure[CDF of average waiting times for all wide jobs]{
\vspace{-0.2in}
	\includegraphics[width=0.31\textwidth]{figures/simulation/average_task_waiting_time_2STrace.pdf}
	%\includegraphics[width=0.31\textwidth]{figures/simulation/task_waiting_time_cdf_JOB-181.pdf}
	\label{fig:sim:waitingTimesTrial:2STrace:same}
	\vspace{-0.1in}
}
	\subfigure[CDF of ratio of waiting times for all wide jobs]{
	\includegraphics[width=0.31\textwidth]{figures/simulation/ratio_task_waiting_time_2STrace.pdf}
	%\includegraphics[width=0.31\textwidth]{figures/simulation/task_waiting_time_cdf_JOB-781.pdf}
	\label{fig:sim:waitingTimesTrial:2STrace:improvement}
	\vspace{-0.1in}
}
\vspace{-0.2in}
\caption{Waiting times for jobs in 2STrace - \updated{2S - 12th May 2020}}
\label{fig:sim:waitingTimesTrial}
\vspace{-0.1in}
\end{figure*}
\questionaj{Refer to fig \ref{fig:sim:waitingTimesTrial} and finalize one among the three variants for task waiting time CDF.}
\fi


  % (thinlimit for the 2STrace is 6 and for the GTrace 3.)}
%Since we assign 5\% of tasks as
%sampling tasks so, the jobs with atleast 30 tasks in total will have atleast 2
%sampling tasks. 
%        In particular, we show results only for jobs with more than 5 tasks in
%        this experiment.
%\questionaj{I am not sure how to justify using 5\% tasks for sampling here
%without refering to the table \ref{table:sim:numPilots}. Please help.}
%We used 3Sigma-Predict with default settings described in 3Sigma and used all
%possible, "expert" pairs recommended. 

%    To make this article self-contained, we briefly describe
%    the scheme here. \primarybasepredict is a distribution based prediction scheme
%    that predicts the historical distribution of runtimes instead of just a point
%    estimate.

%To make this article self-contained we briefly describe it here. It uses four
%estimation techniques namely, average, median, rolling average and average of
%X(=20) recent job runtimes and it uses following features, application name,
%user name, job name, resource requested and submission time (hour, day etc.) of
%the job.  The \primarybasepredict tracks accuracy of each, feature value and
%estimation pair technique \cite{3Sigma} by the help of a running metric. It
%always uses the pair which is expected to give the most accurate prediction.

%%%% Above from simulation.tex on Sep 17 2020 %%%%


==> related.tex <==
\section{Related Work}
\label{sec:related}

We already summarize previous work on history-based learning schemes
and job schedulers in \S\ref{sec:back:existing}. Here we summarize
additioal related work.

\textbf{Job scheduling:}
{Stratus~\cite{stratus:socc2018} is a cluster scheduler that focuses
on optimizing the dollar cost. It uses a runtime predictor
derived from JamiasVu~\cite{jamiasvu} which has feature selection mechanisms
similar to that used in 3Sigma~\cite{3Sigma}.}

The Kairos~\cite{kairos:socc2018} scheduler is built on the principle
  of Least Attained Service.  The policy is inherently preemptive and
  does not provide same liveness guarantee as \slearn with
  \gs. Further, \slearn is a learning based technique and Kairos
  is a non-learning approach.

%  We tried to access the soruce code of Kairos at the
%  url~\cite{kairosScheduler} provided in the paper, but we got a not found error.
%  We also wrote to the author however did not hear back till the time of writing
%  this article.  

\if 0
There have been much work on scheduling in analytic
systems and storage at scale by improving speculative tasks~\cite{late:osdi08,
mantri:OSDI2010, dolly:nsdi13}, improving locality~\cite{delay:eurosys10,
scarlett:eurosys11}, and end-point flexibility~\cite{sinbad:sigcomm13,
  pisces:osdi12}.
 
\fi
\textbf{Speculative scheduling:} Recent works
(\cite{creditscheduling:sigcomm17, trumpet:sigcomm16}) use the idea of
online requirement estimation for scheduling in datacenter.
%In Corral ~\cite{corral}, recurring big data %analytics jobs are scheduled using their history.\\

%  \textbf{Flow scheduling:} There have been a rich body of prior work on flow
%  scheduling to minimize flow completion time, both with prior information (\eg
%  PDQ~\cite{pdq:sigcomm12}, pFabric~\cite{pfabric:sigcomm13}) and without prior
%  information (\eg Fastpass~\cite{fastpass:sigcomm14},
%  PIAS~\cite{pias:hotnets14}, ~\cite{pias:nsdi15}). These problems are
%  orthogonal to the problem discussed in this paper. 

\if 0
{\textbf{Coflow scheduling:} Recent works,
  Graviton~\cite{graviton:hotcloud16} and Saath~\cite{jajooSaath}, in
  coflow scheduling have also exploited the spatial dimension to come
  up with efficient coflow scheduling algorithm.}
\fi
\addnsdiSHP{\textbf{GPU Cluster Scheduling:}
Some recent work use the characteristics of completed mini-batches as 
a proxy for the remaining mini-batches, to improve the scheduling of ML jobs \cite{gandiva:osdi18}.
However, such jobs are different in that the mini-batches in general experience 
significantly less (task-level) variations than what we studied in this paper.}{C4}

==> testbed.tex <==
%\section{Testbed}
%\label{sec:testbed}
Fig. \S\ref{fig:testbed:jctSpeedup3Sigma} shows speedup of \name over \primarybase.
\begin{figure}[tp]
\centering
\includegraphics[width=0.9\linewidth]{figures/testbed/result_analysis-testbed-gTrace-durComp50-Patience-3Sigma-speedUp-CDF.pdf}
\vspace{-0.1in}
	\caption{(Testbed) CDF of JCT speedup of \name over \primarybase on the GTrace.}
\label{fig:testbed:jctSpeedup3Sigma}
\vspace{-0.2in}
\end{figure}

